Towards Machine Learning for Placement and Routing in Chip Design: a Methodological Overview

Placement and routing are two indispensable and challenging (NP-hard) tasks in modern chip design flows. Compared with traditional solvers using heuristics or expert-well-designed algorithms, machine learning has shown promising prospects by its data-driven nature, which can be of less reliance on knowledge and priors, and potentially more scalable by its advanced computational paradigms (e.g. deep networks with GPU acceleration). This survey starts with the introduction of basics of placement and routing, with a brief description on classic learning-free solvers. Then we present detailed review on recent advance in machine learning for placement and routing. Finally we discuss the challenges and opportunities for future research.

==> eda_ref_full.tex <==
@string{TCAD={TCAD}}
@string{DAC={DAC}}
@string{ISPD={ISPD}}
@string{ICCD={ICCD}}
@string{ISNE={ISNE}}
@string{ICCAD={ICCAD}}
@string{ASP-DAC={ASP-DAC}}
@string{NeurIPS={NeurIPS}}
@string{VLSI-DAT={VLSI-DAT}}
@string{Nature={Nature}}


@article{nam2007ispd,
  title={{{ISPD}} 2007 {{Global Routing Contest}}},
  author={Nam, Gi-Joon and Yildiz, Mehmet and Pan, David and Madden, Patrick},
  year={2007}
}

@inproceedings{nam2008ispd,
  title={The ISPD global routing benchmark suite},
  author={Nam, Gi-Joon and Sze, Cliff and Yildiz, Mehmet},
  booktitle={ISPD},
  year={2008}
}

@article{ozdal2009archer,
  title={Archer: A history-based global routing algorithm},
  author={Ozdal, Muhammet Mustafa and Wong, Martin DF},
  journal={TCAD},
  year={2009},
  publisher={IEEE}
}

@article{cho2009boxrouter,
  title={BoxRouter 2.0: A hybrid and robust global router with layer assignment for routability},
  author={Cho, Minsik and Lu, Katrina and Yuan, Kun and Pan, David Z},
  journal={TODAES},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@inproceedings{zhang2008fastroute3,
  title={FastRoute3. 0: a fast and high quality global router based on virtual capacity},
  author={Zhang, Yanheng and Xu, Yue and Chu, Chris},
  booktitle={ICCAD},
  year={2008},
  organization={IEEE}
}

@inproceedings{xu2009fastroute,
  title={FastRoute 4.0: Global router with efficient via minimization},
  author={Xu, Yue and Zhang, Yanheng and Chu, Chris},
  booktitle={ASP-DAC},
  year={2009},
  organization={IEEE}
}

@article{pan2012fastroute,
  title={FastRoute: An efficient and high-quality global router},
  author={Pan, Min and Xu, Yue and Zhang, Yanheng and Chu, Chris},
  journal={VLSI Design},
  year={2012},
  publisher={Hindawi}
}

@article{roy2008high,
  title={High-performance routing at the nanometer scale},
  author={Roy, Jarrod A and Markov, Igor L},
  journal={TCAD},
  year={2008},
  publisher={IEEE}
}

@inproceedings{gao2008new,
  title={A new global router for modern designs},
  author={Gao, Jhih-Rong and Wu, Pei-Ci and Wang, Ting-Chi},
  booktitle={ASP-DAC},
  year={2008},
  organization={IEEE}
}

@inproceedings{wu2009grip,
  title={GRIP: Scalable 3D global routing using integer programming},
  author={Wu, Tai-Hsuan and Davoodi, Azadeh and Linderoth, Jeffrey T},
  booktitle={DAC},
  year={2009}
}

@article{moffitt2008maizerouter,
  title={MaizeRouter: Engineering an effective global router},
  author={Moffitt, Michael D},
  journal={TCAD},
  year={2008},
  publisher={IEEE}
}

@inproceedings{dai2009efficient,
  title={Efficient simulated evolution based rerouting and congestion-relaxed layer assignment on 3-D global routing},
  author={Dai, Ke-Ren and Liu, Wen-Hao and Li, Yih-Lang},
  booktitle={ASP-DAC},
  year={2009},
  organization={IEEE}
}

@article{chang2010nthu,
  title={NTHU-Route 2.0: a robust global router for modern designs},
  author={Chang, Yen-Jung and Lee, Yu-Ting and Gao, Jhih-Rong and Wu, Pei-Ci and Wang, Ting-Chi},
  journal={TCAD},
  year={2010},
  publisher={IEEE}
}

@inproceedings{chen2009high,
  title={High-performance global routing with fast overflow reduction},
  author={Chen, Huang-Yu and Hsu, Chin-Hsiung and Chang, Yao-Wen},
  booktitle={ASP-DAC},
  year={2009},
  organization={IEEE}
}

@article{albrecht2001global,
  title={Global routing by new approximation algorithms for multicommodity flow},
  author={Albrecht, Christoph},
  journal={TCAD},
  year={2001},
  publisher={IEEE}
}

@article{cho2007boxrouter,
  title={BoxRouter: A new global router based on box expansion and progressive ILP},
  author={Cho, Minsik and Pan, David Z},
  journal={TCAD},
  year={2007},
  publisher={IEEE}
}

@article{lee1961algorithm,
  title={An algorithm for path connections and its applications},
  author={Lee, Chin Yang},
  journal={IRE Transactions on Electronic Computers},
  year={1961},
  publisher={IEEE}
}

@article{kastner2002pattern,
  title={Pattern routing: Use and theory for increasing predictability and avoiding coupling},
  author={Kastner, Ryan and Bozorgzadeh, Elaheh and Sarrafzadeh, Majid},
  journal={TCAD},
  year={2002},
  publisher={IEEE}
}

@article{liu2013nctu,
  title={NCTU-GR 2.0: Multithreaded collision-aware global routing with bounded-length maze routing},
  author={Liu, Wen-Hao and Kao, Wei-Chun and Li, Yih-Lang and Chao, Kai-Yuan},
  journal={TCAD},
  year={2013},
  publisher={IEEE}
}

@article{chu2007flute,
  title={FLUTE: Fast lookup table based rectilinear Steiner minimal tree algorithm for VLSI design},
  author={Chu, Chris and Wong, Yiu-Chung},
  journal={TCAD},
  year={2007},
  publisher={IEEE}
}

@inproceedings{zhou2019supervised,
  title={Supervised-learning congestion predictor for routability-driven global routing},
  author={Zhou, Zhonghua and Chahal, Sunmeet and Ho, Tsung-Yi and Ivanov, Andr{\'e}},
  booktitle={VLSI-DAT},
  year={2019},
  organization={IEEE}
}

@inproceedings{chan2016beol,
  title={BEOL stack-aware routability prediction from placement using data mining techniques},
  author={Chan, Wei-Ting J and Du, Yang and Kahng, Andrew B and Nath, Siddhartha and Samadi, Kambiz},
  booktitle={ICCD},
  year={2016},
  organization={IEEE}
}

@inproceedings{cheng2018evaluation,
  title={Evaluation of routability-driven macro placement with machine-learning technique},
  author={Cheng, Wei-Kai and Guo, Yu-Yin and Wu, Chih-Shuan},
  booktitle={ISNE},
  year={2018},
  organization={IEEE}
}

@inproceedings{RESTDAC21,
  title={REST: Constructing Rectilinear Steiner Minimum Tree via Reinforcement Learning},
  author={Jinwei Liu and Gengjie Chen and Evangeline F.Y. Young},
  booktitle={DAC},
  year={2021}
}
@inproceedings{MixedICCAD10,
  title={Design-Hierarchy Aware Mixed-Size Placement for Routability Optimization},
  author={Yi-Lin Chuang and Gi-Joon Nam and Charles J. Alpert and Yao-Wen Chang and Jarrod Roy and Natarajan Viswanathan},
  booktitle={ICCAD},
  year={2010}
}




@inproceedings{breuer1977class,
  title={A class of min-cut placement algorithms},
  author={Breuer, Melvin A},
  booktitle={DAC},
  year={1977}
}

@inproceedings{fiduccia1982linear,
  title={A linear-time heuristic for improving network partitions},
  author={Fiduccia, Charles M and Mattheyses, Robert M},
  booktitle={DAC},
  year={1982},
  organization={IEEE}
}

@inproceedings{agnihotri2005recursive,
  title={Recursive bisection placement: Feng Shui 5.0 implementation details},
  author={Agnihotri, Ameya R and Ono, Satoshi and Madden, Patrick H},
  booktitle={ISPD},
  year={2005}
}

@article{kirkpatrick1983optimization,
  title={Optimization by simulated annealing},
  author={Kirkpatrick, Scott and Gelatt, C Daniel and Vecchi, Mario P},
  journal={Science},
  year={1983},
  publisher={American association for the advancement of science}
}

@article{ho2004orthogonal,
  title={An orthogonal simulated annealing algorithm for large floorplanning problems},
  author={Ho, Shinn-Ying and Ho, Shinn-Jang and Lin, Yi-Kuang and Chu, WC-C},
  journal={VLSI Systems},
  year={2004},
  publisher={IEEE}
}

@article{shunmugathammal2020novel,
  title={A novel B* tree crossover-based simulated annealing algorithm for combinatorial optimization in VLSI fixed-outline floorplans},
  author={Shunmugathammal, M and Columbus, C Christopher and Anand, S},
  journal={Circuits, Systems, and Signal Processing},
  year={2020},
  publisher={Springer}
}

@article{spindler2008kraftwerk2,
  title={Kraftwerk2—A fast force-directed quadratic placement approach using an accurate net model},
  author={Spindler, Peter and Schlichtmann, Ulf and Johannes, Frank M},
  journal={TCAD},
  year={2008},
  publisher={IEEE}
}

@article{chen2008ntuplace3,
  title={NTUplace3: An analytical placer for large-scale mixed-size designs with preplaced blocks and density constraints},
  author={Chen, Tung-Chieh and Jiang, Zhe-Wei and Hsu, Tien-Chang and Chen, Hsin-Chen and Chang, Yao-Wen},
  journal={TCAD},
  year={2008},
  publisher={IEEE}
}

@article{kahng2005implementation,
  title={Implementation and extensibility of an analytic placer},
  author={Kahng, Andrew B and Wang, Qinke},
  journal={TCAD},
  year={2005},
  publisher={IEEE}
}

@article{lu2015eplace,
  title={ePlace: Electrostatics-based placement using fast fourier transform and Nesterov's method},
  author={Lu, Jingwei and Chen, Pengwen and Chang, Chin-Chih and Sha, Lu and Huang, Dennis Jen-Hsin and Teng, Chin-Chi and Cheng, Chung-Kuan},
  journal={TODAES},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@article{cheng2018replace,
  title={Replace: Advancing solution quality and routability validation in global placement},
  author={Cheng, Chung-Kuan and Kahng, Andrew B and Kang, Ilgweon and Wang, Lutong},
  journal={TCAD},
  year={2018},
  publisher={IEEE}
}

@article{lin2020dreamplace,
  title={Dreamplace: Deep learning toolkit-enabled gpu acceleration for modern vlsi placement},
  author={Lin, Yibo and Jiang, Zixuan and Gu, Jiaqi and Li, Wuxi and Dhar, Shounak and Ren, Haoxing and Khailany, Brucek and Pan, David Z},
  journal={TCAD},
  year={2020},
  publisher={IEEE}
}

@article{cheng2021joint,
  title={On Joint Learning for Solving Placement and Routing in Chip Design},
  author={Cheng, Ruoyu and Yan, Junchi},
  journal={NeurIPS},
  year={2021}
}

@article{mirhoseini2021graph,
  title={A graph placement methodology for fast chip design},
  author={Mirhoseini, Azalia and Goldie, Anna and Yazgan, Mustafa and Jiang, Joe Wenjie and Songhori, Ebrahim and Wang, Shen and Lee, Young-Joon and Johnson, Eric and Pathak, Omkar and Nazi, Azade and others},
  journal={Nature},
  year={2021},
  publisher={Nature Publishing Group}
}

@inproceedings{wu2010parallel,
  title={A parallel integer programming approach to global routing},
  author={Wu, Tai-Hsuan and Davoodi, Azadeh and Linderoth, Jeffrey T},
  booktitle={DAC},
  year={2010},
  organization={IEEE}
}

@article{liao2020deep,
  title={A deep reinforcement learning approach for global routing},
  author={Liao, Haiguang and Zhang, Wentai and Dong, Xuliang and Poczos, Barnabas and Shimada, Kenji and Burak Kara, Levent},
  journal={Journal of Mechanical Design},
  year={2020},
  publisher={American Society of Mechanical Engineers}
}

@inproceedings{liao2020attention,
  title={Attention Routing: track-assignment detailed routing using attention-based reinforcement learning},
  author={Liao, Haiguang and Dong, Qingyi and Dong, Xuliang and Zhang, Wentai and Zhang, Wangyang and Qi, Weiyi and Fallon, Elias and Kara, Levent Burak},
  booktitle={International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
  year={2020},
  organization={American Society of Mechanical Engineers}
}

@inproceedings{ren2021standard,
  title={Standard Cell Routing with Reinforcement Learning and Genetic Algorithm in Advanced Technology Nodes},
  author={Ren, Haoxing and Fojtik, Matthew},
  booktitle={ASP-DAC},
  year={2021}
}

@inproceedings{utyamishev2020late,
  title={Late Breaking Results: A Neural Network that Routes ICs},
  author={Utyamishev, Dmitry and Partin-Vaisband, Inna},
  booktitle={DAC},
  year={2020},
  organization={IEEE}
}

@article{kramer1984complexity,
  title={The complexity of wirerouting and finding minimum area layouts for arbitrary VLSI circuits},
  author={Kramer, Mark R},
  journal={Advances in Computing Research},
  year={1984},
  publisher={JAI press}
}


@inproceedings{xie2018routenet,
  title={RouteNet: Routability prediction for mixed-size designs using convolutional neural network},
  author={Xie, Zhiyao and Huang, Yu-Hung and Fang, Guan-Qi and Ren, Haoxing and Fang, Shao-Yun and Chen, Yiran and Hu, Jiang},
  booktitle={ICCAD},
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@inproceedings{chen2020pros,
  title={PROS: A plug-in for routability optimization applied in the state-of-the-art commercial EDA tool using deep learning},
  author={Chen, Jingsong and Kuang, Jian and Zhao, Guowei and Huang, Dennis J-H and Young, Evangeline FY},
  booktitle={ICCAD},
  year={2020},
  organization={IEEE}
}

@inproceedings{liang2020drc,
  title={DRC hotspot prediction at sub-10nm process nodes using customized convolutional network},
  author={Liang, Rongjian and Xiang, Hua and Pandey, Diwesh and Reddy, Lakshmi and Ramji, Shyam and Nam, Gi-Joon and Hu, Jiang},
  booktitle={ISPD},
  year={2020}
}

@inproceedings{pui2017clock,
  title={Clock-aware ultrascale FPGA placement with machine learning routability prediction},
  author={Pui, Chak-Wa and Chen, Gengjie and Ma, Yuzhe and Young, Evangeline FY and Yu, Bei},
  booktitle={ICCAD},
  year={2017},
  organization={IEEE}
}

@inproceedings{alawieh2020high,
  title={High-definition routing congestion prediction for large-scale FPGAs},
  author={Alawieh, Mohamed Baker and Li, Wuxi and Lin, Yibo and Singhal, Love and Iyer, Mahesh A and Pan, David Z},
  booktitle={ASP-DAC},
  year={2020},
  organization={IEEE}
}

@inproceedings{cheng2018evaluation,
  title={Evaluation of routability-driven macro placement with machine-learning technique},
  author={Cheng, Wei-Kai and Guo, Yu-Yin and Wu, Chih-Shuan},
  booktitle={ISNE},
  year={2018},
  organization={IEEE}
}

@inproceedings{maarouf2018machine,
  title={Machine-learning based congestion estimation for modern FPGAs},
  author={Maarouf, Dani and Alhyari, Abeer and Abuowaimer, Ziad and Martin, Timothy and Gunter, Andrew and Gr{\'e}wal, Gary and Areibi, Shawki and Vannelli, Anthony},
  booktitle={2018 28th International Conference on Field Programmable Logic and Applications (FPL)},
  year={2018},
  organization={IEEE}
}

@inproceedings{qi2014accurate,
  title={Accurate prediction of detailed routing congestion using supervised data learning},
  author={Qi, Zhongdong and Cai, Yici and Zhou, Qiang},
  booktitle={ICCD},
  year={2014},
  organization={IEEE}
}

@inproceedings{zhou2015accurate,
  title={An accurate detailed routing routability prediction model in placement},
  author={Zhou, Quan and Wang, Xueyan and Qi, Zhongdong and Chen, Zhuwei and Zhou, Qiang and Cai, Yici},
  booktitle={2015 6th Asia Symposium on Quality Electronic Design (ASQED)},
  year={2015},
  organization={IEEE}
}

@inproceedings{liu2021global,
  title={Global placement with deep learning-enabled explicit routability optimization},
  author={Liu, Siting and Sun, Qi and Liao, Peiyu and Lin, Yibo and Yu, Bei},
  booktitle={2021 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
  year={2021},
  organization={IEEE}
}

@inproceedings{yu2019painting,
  title={Painting on placement: Forecasting routing congestion using conditional generative adversarial nets},
  author={Yu, Cunxi and Zhang, Zhiru},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@article{al2021deep,
  title={A deep learning framework to predict routability for FPGA circuit placement},
  author={Al-Hyari, Abeer and Szentimrey, Hannah and Shamli, Ahmed and Martin, Timothy and Gr{\'e}wal, Gary and Areibi, Shawki},
  journal={ACM Transactions on Reconfigurable Technology and Systems (TRETS)},
  year={2021},
  publisher={ACM New York, NY}
}

@inproceedings{tabrizi2018machine,
  title={A machine learning framework to identify detailed routing short violations from a placed netlist},
  author={Tabrizi, Aysa Fakheri and Rakai, Logan and Darav, Nima Karimpour and Bustany, Ismail and Behjat, Laleh and Xu, Shuchang and Kennings, Andrew},
  booktitle={DAC},
  year={2018},
  organization={IEEE}
}

@article{jain2017training,
  title={Training a fully convolutional neural network to route integrated Circuits},
  author={Jain, Sambhav R and Okabe, Kye},
  journal={arXiv preprint arXiv:1706.08948},
  year={2017}
}

@article{he2020circuit,
  title={Circuit routing using monte carlo tree search and deep neural networks},
  author={He, Youbiao and Bao, Forrest Sheng},
  journal={arXiv preprint arXiv:2006.13607},
  year={2020}
}

@inproceedings{breuer1977class,
  title={A class of min-cut placement algorithms},
  author={Breuer, Melvin A},
  booktitle={Proceedings of the 14th Design Automation Conference},
  pages={284--290},
  year={1977}
}

@inproceedings{fiduccia1982linear,
  title={A linear-time heuristic for improving network partitions},
  author={Fiduccia, Charles M and Mattheyses, Robert M},
  booktitle={19th design automation conference},
  pages={175--181},
  year={1982},
  organization={IEEE}
}

@inproceedings{agnihotri2005recursive,
  title={Recursive bisection placement: Feng Shui 5.0 implementation details},
  author={Agnihotri, Ameya R and Ono, Satoshi and Madden, Patrick H},
  booktitle={Proceedings of the 2005 international symposium on Physical design},
  pages={230--232},
  year={2005}
}

@article{kirkpatrick1983optimization,
  title={Optimization by simulated annealing},
  author={Kirkpatrick, Scott and Gelatt, C Daniel and Vecchi, Mario P},
  journal={science},
  volume={220},
  number={4598},
  pages={671--680},
  year={1983},
  publisher={American association for the advancement of science}
}

@article{ho2004orthogonal,
  title={An orthogonal simulated annealing algorithm for large floorplanning problems},
  author={Ho, Shinn-Ying and Ho, Shinn-Jang and Lin, Yi-Kuang and Chu, WC-C},
  journal={IEEE transactions on very large scale integration (VLSI) systems},
  volume={12},
  number={8},
  pages={874--877},
  year={2004},
  publisher={IEEE}
}

@article{shunmugathammal2020novel,
  title={A novel B* tree crossover-based simulated annealing algorithm for combinatorial optimization in VLSI fixed-outline floorplans},
  author={Shunmugathammal, M and Columbus, C Christopher and Anand, S},
  journal={Circuits, Systems, and Signal Processing},
  volume={39},
  number={2},
  pages={900--918},
  year={2020},
  publisher={Springer}
}

@article{lu2015eplace,
  title={ePlace: Electrostatics-based placement using fast fourier transform and Nesterov's method},
  author={Lu, Jingwei and Chen, Pengwen and Chang, Chin-Chih and Sha, Lu and Huang, Dennis Jen-Hsin and Teng, Chin-Chi and Cheng, Chung-Kuan},
  journal={ACM Transactions on Design Automation of Electronic Systems (TODAES)},
  volume={20},
  number={2},
  pages={1--34},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@article{cheng2018replace,
  title={Replace: Advancing solution quality and routability validation in global placement},
  author={Cheng, Chung-Kuan and Kahng, Andrew B and Kang, Ilgweon and Wang, Lutong},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={38},
  number={9},
  pages={1717--1730},
  year={2018},
  publisher={IEEE}
}

@article{spindler2008kraftwerk2,
  title={Kraftwerk2—A fast force-directed quadratic placement approach using an accurate net model},
  author={Spindler, Peter and Schlichtmann, Ulf and Johannes, Frank M},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={27},
  number={8},
  pages={1398--1411},
  year={2008},
  publisher={IEEE}
}

@article{chen2008ntuplace3,
  title={NTUplace3: An analytical placer for large-scale mixed-size designs with preplaced blocks and density constraints},
  author={Chen, Tung-Chieh and Jiang, Zhe-Wei and Hsu, Tien-Chang and Chen, Hsin-Chen and Chang, Yao-Wen},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={27},
  number={7},
  pages={1228--1240},
  year={2008},
  publisher={IEEE}
}

@article{vashisht2020placement,
  title={Placement in Integrated Circuits using Cyclic Reinforcement Learning and Simulated Annealing},
  author={Vashisht, Dhruv and Rampal, Harshit and Liao, Haiguang and Lu, Yang and Shanbhag, Devika and Fallon, Elias and Kara, Levent Burak},
  journal={arXiv preprint arXiv:2011.07577},
  year={2020}
}

@article{caldwell2000optimal,
  title={Optimal partitioners and end-case placers for standard-cell layout},
  author={Caldwell, Andrew E and Kahng, Andrew B and Markov, Igor L},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={19},
  number={11},
  pages={1304--1313},
  year={2000},
  publisher={IEEE}
}

@article{kahng2005implementation,
  title={Implementation and extensibility of an analytic placer},
  author={Kahng, Andrew B and Wang, Qinke},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={24},
  number={5},
  pages={734--747},
  year={2005},
  publisher={IEEE}
}

@inproceedings{alpert2010makes,
  title={What makes a design difficult to route},
  author={Alpert, Charles J and Li, Zhuo and Moffitt, Michael D and Nam, Gi-Joon and Roy, Jarrod A and Tellez, Gustavo},
  booktitle={Proceedings of the 19th international symposium on Physical design},
  pages={7--12},
  year={2010}
}

@inproceedings{kim2011simplr,
  title={A SimPLR method for routability-driven placement},
  author={Kim, Myung-Chul and Hu, Jin and Lee, Dong-Jin and Markov, Igor L},
  booktitle={2011 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
  pages={67--73},
  year={2011},
  organization={IEEE}
}

@inproceedings{hsu2011routability,
  title={Routability-driven analytical placement for mixed-size circuit designs},
  author={Hsu, Meng-Kai and Chou, Sheng and Lin, Tzu-Hen and Chang, Yao-Wen},
  booktitle={2011 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
  pages={80--84},
  year={2011},
  organization={IEEE}
}

@inproceedings{luo2006new,
  title={A new LP based incremental timing driven placement for high performance designs},
  author={Luo, Tao and Newmark, David and Pan, David Z},
  booktitle={Proceedings of the 43rd annual Design Automation Conference},
  pages={1115--1120},
  year={2006}
}

@article{lee2012obstacle,
  title={Obstacle-aware clock-tree shaping during placement},
  author={Lee, Dong-Jin and Markov, Igor L},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={31},
  number={2},
  pages={205--216},
  year={2012},
  publisher={IEEE}
}

@inproceedings{cheon2005power,
  title={Power-aware placement},
  author={Cheon, Yongseok and Ho, Pei-Hsin and Kahng, Andrew B and Reda, Sherief and Wang, Qinke},
  booktitle={Proceedings of the 42nd annual Design Automation Conference},
  pages={795--800},
  year={2005}
}

@inproceedings{riess1995speed,
  title={Speed: Fast and efficient timing driven placement},
  author={Riess, Bernhard M and Ettelt, Gisela G},
  booktitle={Proceedings of ISCAS'95-International Symposium on Circuits and Systems},
  volume={1},
  pages={377--380},
  year={1995},
  organization={IEEE}
}

@article{huang2021machine,
  title={Machine learning for electronic design automation: A survey},
  author={Huang, Guyue and Hu, Jingbo and He, Yifan and Liu, Jialong and Ma, Mingyuan and Shen, Zhaoyang and Wu, Juejian and Xu, Yuanfan and Zhang, Hengrui and Zhong, Kai and others},
  journal={ACM Transactions on Design Automation of Electronic Systems (TODAES)},
  volume={26},
  number={5},
  pages={1--46},
  year={2021},
  publisher={ACM New York, NY}
}

@article{mirhoseini2021graph,
  title={A graph placement methodology for fast chip design},
  author={Mirhoseini, Azalia and Goldie, Anna and Yazgan, Mustafa and Jiang, Joe Wenjie and Songhori, Ebrahim and Wang, Shen and Lee, Young-Joon and Johnson, Eric and Pathak, Omkar and Nazi, Azade and others},
  journal={Nature},
  volume={594},
  number={7862},
  pages={207--212},
  year={2021},
  publisher={Nature Publishing Group}
}

@inproceedings{he2020learn,
  title={Learn to floorplan through acquisition of effective local search heuristics},
  author={He, Zhuolun and Ma, Yuzhe and Zhang, Lu and Liao, Peiyu and Wong, Ngai and Yu, Bei and Wong, Martin DF},
  booktitle={2020 IEEE 38th International Conference on Computer Design (ICCD)},
  pages={324--331},
  year={2020},
  organization={IEEE}
}

@article{cheng2021joint,
  title={On Joint Learning for Solving Placement and Routing in Chip Design},
  author={Cheng, Ruoyu and Yan, Junchi},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@article{lin2020dreamplace,
  title={Dreamplace: Deep learning toolkit-enabled gpu acceleration for modern vlsi placement},
  author={Lin, Yibo and Jiang, Zixuan and Gu, Jiaqi and Li, Wuxi and Dhar, Shounak and Ren, Haoxing and Khailany, Brucek and Pan, David Z},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  year={2020},
  publisher={IEEE}
}

@inproceedings{lu2021law,
  title={The law of attraction: Affinity-aware placement optimization using graph neural networks},
  author={Lu, Yi-Chen and Pentapati, Sai and Lim, Sung Kyu},
  booktitle={Proceedings of the 2021 International Symposium on Physical Design},
  pages={7--14},
  year={2021}
}

@inproceedings{ward2012pade,
  title={PADE: A high-performance placer with automatic datapath extraction and evaluation through high-dimensional data learning},
  author={Ward, Samuel and Ding, Duo and Pan, David Z},
  booktitle={DAC Design Automation Conference 2012},
  pages={756--761},
  year={2012},
  organization={IEEE}
}

@inproceedings{li2021learning,
  title={Learning Point Clouds in EDA},
  author={Li, Wei and Chen, Guojin and Yang, Haoyu and Chen, Ran and Yu, Bei},
  booktitle={Proceedings of the 2021 International Symposium on Physical Design},
  pages={55--62},
  year={2021}
}

@article{li2022adaptive,
  title={Adaptive layout decomposition with graph embedding neural networks},
  author={Li, Wei and Ma, Yuzhe and Lin, Yibo and Yu, Bei},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  year={2022},
  publisher={IEEE}
}

@inproceedings{zhang2020grannite,
  title={GRANNITE: Graph neural network inference for transferable power estimation},
  author={Zhang, Yanqing and Ren, Haoxing and Khailany, Brucek},
  booktitle={2020 57th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@inproceedings{wang2020gcn,
  title={GCN-RL circuit designer: Transferable transistor sizing with graph neural networks and reinforcement learning},
  author={Wang, Hanrui and Wang, Kuan and Yang, Jiacheng and Shen, Linxiao and Sun, Nan and Lee, Hae-Seung and Han, Song},
  booktitle={2020 57th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@inproceedings{huang2019routability,
  title={Routability-driven macro placement with embedded CNN-based prediction model},
  author={Huang, Yu-Hung and Xie, Zhiyao and Fang, Guan-Qi and Yu, Tao-Chun and Ren, Haoxing and Fang, Shao-Yun and Chen, Yiran and Hu, Jiang},
  booktitle={2019 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
  pages={180--185},
  year={2019},
  organization={IEEE}
}

@inproceedings{chan2017routability,
  title={Routability optimization for industrial designs at sub-14nm process nodes using machine learning},
  author={Chan, Wei-Ting J and Ho, Pei-Hsin and Kahng, Andrew B and Saxena, Prashant},
  booktitle={Proceedings of the 2017 ACM on International Symposium on Physical Design},
  pages={15--21},
  year={2017}
}

